Computational Design of Active Kinesthetic Garments

Garments with the ability to provide kinesthetic force-feedback on-demand can augment human capabilities in a non-obtrusive way, enabling numerous applications in VR haptics, motion assistance, and robotic control. However, designing such garments is a complex, and often manual task, particularly when the goal is to resist multiple motions with a single design. In this work, we propose a computational pipeline for designing connecting structures between active components - one of the central challenges in this context. We focus on electrostatic (ES) clutches that are compliant in their passive state while strongly resisting elongation when activated. Our method automatically computes optimized connecting structures that efficiently resist a range of pre-defined body motions on demand. We propose a novel dual-objective optimization approach to simultaneously maximize the resistance to motion when clutches are active, while minimizing resistance when inactive. We demonstrate our method on a set of problems involving different body sites and a range of motions. We further fabricate and evaluate a subset of our automatically created designs against manually created baselines using mechanical testing and in a VR pointing study.

==> other/commands.tex <==
% vectors, matrices, sets, and functions
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mat}[1]{\boldsymbol{\mathrm{#1}}}
\let\set=\mathcal
\let\func=\mathrm

% common symbols
\newcommand{\N}{\mbox{\rm \hbox{I\kern-.15em\hbox{N}}}}
\newcommand{\R}{\mbox{\rm \hbox{I\kern-.15em\hbox{R}}}}
\newcommand{\laplace}{\Delta}
\newcommand{\grad}{\nabla}
\newcommand{\strain}{\vec{\epsilon}}
\newcommand{\stress}{\vec{\sigma}}

\newcommand{\minipar}[1]{\vspace{.75ex}\noindent\textbf{#1}\hspace{2ex}}

%\renewcommand{\SS}{{\mathcal{E}}}
\newcommand{\RS}{{\mathcal{F}}}
\newcommand{\ES}{{\mathcal{E}}}

% some math commands
\def \N {\mbox{\rm \hbox{I\kern-.15em\hbox{N}}}}
\def \R {\mbox{\rm \hbox{I\kern-.15em\hbox{R}}}}
\def \laplace {\Delta}
\def \grad {\nabla}
\def \dprod {\mspace{-1mu} \cdot \mspace{-1mu}}
\def \tprod {\mspace{-1mu} : \mspace{-1mu}}
\newcommand{\of}[1]{\mspace{-3mu}\left( #1 \right)}
\newcommand{\ofx}{\of{\vec{x}}}
%\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\twovec}[2]{\left[\begin{array}{c}#1\\#2\end{array}\right]}
\newcommand{\threevec}[3]{\left[\begin{array}{c}#1\\#2\\#3\end{array}\right]}
\renewcommand{\matrix}[2]{\left[\begin{array}{#1}#2\end{array}\right]}
\newcommand{\dV}{\,\mathrm{d}\Omega}
\newcommand{\dA}{\,\mathrm{d}\set{S}}
\newcommand{\ds}{\,\mathrm{d}\Gamma}

% references and abbreviations
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\Sec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\Equation}[1]{Equation ~(\ref{eq:#1})}
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand{\Appendix}[1]{Appendix~\ref{app:#1}}

%specific commands from the hfem paper
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bmm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bw}{\vec{w}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bZero}{\mathbf{0}}

\newcommand{\energy}{U}
\newcommand{\energydensity}{W}
\newcommand{\materialdensity}{d}
\newcommand{\sensitivity}{\alpha}

\newcommand{\bodyDef}{\mathbf{y}}
\newcommand{\bodyUndef}{\bar{\bodyDef}}
\newcommand{\clothDef}{\mathbf{s}}

%\newcommand{\fint}{\mathbf{f}_\mathrm{int}}
\newcommand{\fext}{\mathbf{f}_\mathrm{ext}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\btheta}{\boldsymbol{\theta}}

\newcommand{\tC}{\mathbb{C}}
\newcommand{\tS}{\mathbb{S}}
\newcommand{\tB}{\mathbb{B}}
\newcommand{\curvature}{\boldsymbol{\kappa}}

\newcommand{\var}{\,\cdot\,}

% \newcommand{\Comment}[3]
% {
% \textcolor{#3}{#1: #2}
% }

%\newcommand{\changed}[1]{\textcolor{red!80!black}{#1}}
\newcommand{\changed}[1]{#1}


==> other/math.tex <==
\newcommand{\SetOfStates}{\mathcal{S}}
\newcommand{\StatePerPolicy}{S}
\newcommand{\NumberOfPlayers}{\mathcal{N}}
\newcommand{\SetOfActions}{\mathcal{A}}
\newcommand{\ActionPerPolicy}{A}
\newcommand{\Transitions}{\mathcal{P}}
\newcommand{\SetOfRewards}{\mathcal{R}}
\newcommand{\RewardPerPolicy}{R}
\newcommand{\SetOfPolicies}{\Pi}
\newcommand{\discount}{\gamma}

\newcommand{\action}{\mathbf{a}}
\renewcommand{\state}{\mathbf{s}}
\newcommand{\policy}{\pi}


\newcommand{\tools}{\mathbf{t}}
\newcommand{\gattr}{\mathbf{g}}
\newcommand{\pos}{\mathbf{p}}
\newcommand{\menu}{\mathbf{m}}

\newcommand{\button}{\mathbf{b}}
\newcommand{\mt}{T_M}
\newcommand{\dect}{T_D}

\newcommand{\taskCompletionTime}{tkt}

==> other/util.tex <==
%********CUSTOM COMMANDS**********%
\usepackage{xcolor}

% create a shortcut to typeset table headings
\newcommand\tabhead[1]{\small\textbf{#1}}

% \definecolor{brown}{rgb}{0.59, 0.29, 0.0}
% \definecolor{darkgray}{rgb}{0.59, 0.59, 0.59}

% COMMANDS FOR NOTES PER PERSON
\newcommand\VV[1]{\textit{\textcolor{orange}{VV:#1}}}
\newcommand\OH[1]{\textit{\textcolor{green}{OH:#1}}}
\newcommand\BT[1]{\textit{\textcolor{yellow}{BT:#1}}}
\newcommand\RH[1]{\textit{\textcolor{red}{RH:#1}}}

% \newcommand\todo[1]{\textit{\textcolor{brown}{[todo]~#1}}}

% REVISIONS Color
\newcommand\REV[1]{\textcolor{black}{#1}}


\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\secref}[1]{the Section~\nameref{#1}}
\newcommand\mydots{\hbox to 1em{.\hss.\hss.}}

%\newcommand\david[1]{}
%\newcommand\otmar[1]{}
\newcommand\remove[1]{}

%\newcommand{\comment}[1]{}

\usepackage[utf8]{inputenc}

\usepackage{tabularx}
\usepackage[percent]{overpic}

\usepackage{nameref}

\usepackage{hyperref}
\usepackage{url}

\usepackage{xspace}
\usepackage{enumitem}
\usepackage{mathtools}
\usepackage{commath}
\DeclareMathOperator*{\argmin}{argmin}

% \usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{53}}%

\newcommand{\customtilde}{{\raise.17ex\hbox{$\scriptstyle\sim$}}}

\newcommand{\mv}[1]{\mathbf{#1}}
%\def \R {\mathbb{R}}
%\def \Z {\mathbb{Z}}
\def \tp {^{\mathsf{T}}}

\newcommand{\etal}{et~al.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\cf}{cf.\xspace}
\newcommand{\etc}{etc.\xspace}

%\newcommand{\subparagraph}[1]{\textit{{#1}}:~}

%********END CUSTOM COMMANDS**********%

==> sections/abstract.tex <==
%!TEX root = ../main.tex
% Soft robotic garments with the ability to provide actuation and sensing via active components are an emergent technology in the fields of VR haptics, locomotion assistance, robotic control, and many others. However, creating designs for sensor and actuator structures is a difficult task, as they need to consider bodily motion(s), and the non-linear garment-on-body interaction. Our main contribution in this work is a  computational pipeline to address the problem of creating \emph{connecting structures} between active components, in particular, a type of kinesthetic feedback components (ES Clutches). Our pipeline models, simulates, and automatically connects ES clutches with the goal of maximizing an energy differential between when clutches are ON and OFF.  
% We demonstrate our method on a variety of design problems on different body sites under a range of motions. Optimal designs both increase the maximum energy density when clutches are ON and reduce the energy of the system in the OFF state. We show that our method can effectively optimize connecting structures for multiple motions while drastically reducing the material needed to do so. We fabricate and test a subset of our optimal designs, showing improved user performance in a VR study.

Garments with the ability to provide kinesthetic force-feedback on-demand can augment human capabilities in a non-obtrusive way, enabling numerous applications in VR haptics, motion assistance, and robotic control. However, designing such garments is a complex, and often manual task, particularly when the goal is to resist multiple motions with a single design. In this work, we propose a computational pipeline for designing  \emph{connecting structures} between active components---one of the central challenges in this context. We focus on electrostatic (ES) clutches that are compliant in their passive state while strongly resisting elongation when activated. Our method automatically computes optimized connecting structures that efficiently resist a range of pre-defined body motions on demand. We propose a novel dual-objective optimization approach to simultaneously maximize the resistance to motion when clutches are active, while minimizing resistance when inactive. We demonstrate our method on a set of problems involving different body sites and a range of motions. We further fabricate and evaluate a subset of our automatically created designs against manually created baselines using mechanical testing and in a VR pointing study. 

% T


% 1. lets get to the point of what WE do quicker
% 2. then explain what the method does (already there in parts)
% 3. what the user gets
% 4. preview of the results

% Kinesthetic garments provide physical feedback on body posture and motion through tailored distributions of reinforced material. Their ability to selectively stiffen a garment's response to specific motions makes them appealing for rehabilitation, sports, robotics, and many other application fields.
% % Designing kinesthetic garments, however, is a challenging problem.   
% % First, while reinforcements should provide a sufficient level of mechanical feedback, adding too much stiff material will interfere with the original behavior of the garment and degrade its comfort.  
% % Second, due to their nonlinear mechanics and complex relation between body motion and induced garment deformation, predicting the performance of a given design is difficult. Consequently, 
% However, finding designs that distribute a given amount of reinforcement material to maximally stiffen the response to specified motions is a challenging problem. In this work, we propose an optimization-driven approach for automated design of reinforcement patterns for kinesthetic garments. Our main contribution is to cast this design task as an on-body topology optimization problem. Our method allows designers to explore a continuous range of designs corresponding to various amounts of reinforcement coverage. Our model captures both tight contact and lift-off separation between cloth and body. 
% We demonstrate our method on a variety of reinforcement design problems for different body sites and motions. Optimal designs lead to a two- to threefold improvement in performance in terms of energy density. A set of manufactured designs were consistently rated as providing more resistance than baselines in a comparative user study. \\f wf
